Efficient Depth Estimation for Unstable Stereo Camera Systems on AR Glasses

Stereo depth estimation is a fundamental component in augmented reality (AR), which requires low latency for real-time processing. However, preprocessing such as rectification and non-ML computations such as cost volume require significant amount of latency exceeding that of an ML model itself, which hinders the real-time processing required by AR. Therefore, we develop alternative approaches to the rectification and cost volume that consider ML acceleration (GPU and NPUs) in recent hardware. For pre-processing, we eliminate it by introducing homography matrix prediction network with a rectification positional encoding (RPE), which delivers both low latency and robustness to unrectified images. For cost volume, we replace it with a group-pointwise convolution-based operator and approximation of cosine similarity based on layernorm and dot product. Based on our approaches, we develop MultiHeadDepth (replacing cost volume) and HomoDepth (MultiHeadDepth + removing pre-processing) models. MultiHeadDepth provides 11.8-30.3% improvements in accuracy and 22.9-25.2% reduction in latency compared to a state-of-the-art depth estimation model for AR glasses from industry. HomoDepth, which can directly process unrectified images, reduces the end-to-end latency by 44.5%. We also introduce a multi-task learning method to handle misaligned stereo inputs on HomoDepth, which reduces the AbsRel error by 10.0-24.3%. The overall results demonstrate the efficacy of our approaches, which not only reduce the inference latency but also improve the model performance. Our code is available at https://github.com/UCI-ISA-Lab/MultiHeadDepth-HomoDepth

==> algorithms/cost_volume.tex <==

\begin{algorithm}
\small
\caption{Cost Volume}
\label{alg:cost_volume}
\begin{algorithmic}
\Require 
\State $left: [NCHW]$ \Comment{feature map of left image}
\State $right: [NCHW]$ \Comment{feature map of right image}
\State $max\_disparity: int$ \Comment{maximum disparity, generally is 10}
\Ensure 
\State $cost\_volume: [N, max\_disparity, H, W]$

\vspace{3mm} 
\For{$i \in 1:max\_disparity+1$}
    \State $right\_shifted = \text{roll}(right, i)$
    \State $similarity = \text{cosine\_similarity}(left, right\_shifted)$
    \State $cost\_volume[:, i, :, :] = similarity$
\EndFor
\end{algorithmic}
\end{algorithm}

==> figures/homo_rect.tex <==
\begin{figure}[t]
        \centering
        \begin{subfigure}{0.9\linewidth}
            \centering
            \includegraphics[height=0.10\textheight]{figures/org_img.png}
            \caption{\small The original stereo images}
            \label{fig:homo_rect_1}
        \end{subfigure}
        \hfill 

        \begin{subfigure}{0.9\linewidth}
        \centering
            \includegraphics[height=0.093\textheight]{figures/homo_img.png}
            \caption{\small Images after homography matrix-based transformation.}
            \label{fig:homo_rect_2}
        \end{subfigure}
        \vspace{-3mm}
        \caption{\small \textbf{Homography rectification example.} Blue  to indicate margins after transformation.
        }
        \vspace{-2mm}
        \label{fig:homo_rect}
    \end{figure}



==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/ablation.tex <==

\begin{table}
\centering
\resizebox{0.53\textwidth}{!}{%
\begin{tabular}{cccrr|crr|crr|crr}
\hline
\multicolumn{2}{l}{\multirow{2}{*}{}}                                                                                                                  & \multicolumn{3}{c|}{\textbf{Argos}}                                                              & \multicolumn{3}{c|}{\textbf{PreP+Argos}}                                                         & \multicolumn{3}{c|}{\textbf{PreP+MultiHeadDepth}}                                                & \multicolumn{3}{c}{\textbf{HomoDepth}}                                                                   \\ \cline{3-14} 
\multicolumn{2}{l}{}                                                                                                                                   & \textbf{AbsRel}           & \multicolumn{1}{c}{\textbf{D1}} & \multicolumn{1}{c|}{\textbf{RMSE}} & \textbf{AbsRel}           & \multicolumn{1}{c}{\textbf{D1}} & \multicolumn{1}{c|}{\textbf{RMSE}} & \textbf{AbsRel}           & \multicolumn{1}{c}{\textbf{D1}} & \multicolumn{1}{c|}{\textbf{RMSE}} & \textbf{AbsRel}                    & \multicolumn{1}{c}{\textbf{D1}} & \multicolumn{1}{c}{\textbf{RMSE}} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Dataset}}}                                                & \multicolumn{1}{c|}{\textbf{DTU}}              & \multicolumn{1}{r}{0.122} & 0.61                            & 536.91                             & \multicolumn{1}{r}{0.109} & 0.54                            & 210.8                              & \multicolumn{1}{r}{0.099} & \textbf{0.38}                   & \textbf{204.4}                     & \multicolumn{1}{r}{\textbf{0.098}} & \textbf{0.38}                   & 208.8                             \\ \cline{2-14} 
\multicolumn{1}{c|}{}                                                                                 & \multicolumn{1}{c|}{\textbf{DTU\_df}}          & \multicolumn{1}{r}{0.183} & 0.64                            & 599.32                             & \multicolumn{1}{r}{0.115} & 0.55                            & 223.1                              & \multicolumn{1}{r}{0.107} & 0.48                            & 287.8                              & \multicolumn{1}{r}{\textbf{0.087}} & \textbf{0.32}                   & \textbf{184.9}                    \\ \cline{2-14} 
\multicolumn{1}{c|}{}                                                                                 & \multicolumn{1}{l|}{\textbf{Sceneflow\_persp}} & \multicolumn{1}{r}{0.232} & 0.71                            & 597.33                             & \multicolumn{1}{r}{0.121} & 0.43                            & 209.9                              & \multicolumn{1}{r}{0.114} & 0.42                            & 215.3                              & \multicolumn{1}{r}{\textbf{0.097}} & \textbf{0.40}                   & \textbf{198.4}                    \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Latency\\ (ms)\end{tabular}}}} & \multicolumn{1}{c|}{\textbf{CPU}}              & \multicolumn{3}{c|}{811.0}                                                                       & \multicolumn{3}{c|}{1068.3}                                                                      & \multicolumn{3}{c|}{884.4}                                                                       & \multicolumn{3}{c}{\textbf{761.2}}                                                                       \\ \cline{2-14} 
\multicolumn{1}{c|}{}                                                                                 & \multicolumn{1}{c|}{\textbf{GPU}}              & \multicolumn{3}{c|}{109.0}                                                                       & \multicolumn{3}{c|}{312.5}                                                                       & \multicolumn{3}{c|}{312.6}                                                                       & \multicolumn{3}{c}{\textbf{84.5}}                                                                        \\ \hline
\end{tabular}
}
\vspace{-3mm}
\caption{\small \textbf{Ablation study comparing models with or without rectification preprocessing (PreP).} DTU dataset represents a stereo system with a fixed focal length but variable relative position, while DTU\_df represents a system with both variable focal length and position. Sceneflow\_persp is the simulation of bending by perspective transformation.}
\label{tab:ablation}
\vspace{-4mm}
\end{table}

==> tables/data_sum.tex <==
\begin{table*}[ht]
\centering

\footnotesize
\begin{tblr}{
    colspec={|X[1.2,c]|X[4,l]|X[4.5,l]|X[5.1,l]|}, 
    row{1} = {bg=gray!20, fg=black, halign=c}, 
    % rows = {halign=l},
    vlines, 
}
    \hline
    \textbf{Dataset} & \textbf{SceneFlow} & \textbf{DTU} & \textbf{ADT} \\
    \hline
    \textbf{Data Scenario} & 
    The data is rendered from synthetic scenarios, including road driving, flying items, and cartoon characters. & 
    The data is captured using a real camera mounted on a robotic arm, with each frame containing only a single item. & 
    The data is captured by heterogeneous cameras mounted on AR glasses. It contains the users' daily scenarios in the office and apartment. \\
    \hline
    \textbf{Images Quality} & 
    Images captured by synthetic cameras. It provides calibrated RGB images. & 
    Images captured by a real camera. It provides calibrated RGB images. & 
    Images captured by a standard RGB camera and a fisheye grayscale camera. They provide raw RGB and grayscale images. \\
    \hline
    \textbf{Stereo Quality} & 
    Stereo images are rectified. & 
    The robotic arm moves around the target item and takes MVS images. Neighbor image pairs are not rectified. & 
    The cameras are fixed on rigid glass frames and raw stereo images can be rectified. \\
    \hline
    \textbf{Stereo Baseline} & 
    All baselines are 1.0 meters. & 
    Baselines are dynamic, from 7.8 cm to 14.9 cm. & 
    The baselines are rigid at 12.8 cm, which can be considered a standard baseline for AR glasses. \\
    \hline
    \textbf{Depth Map} & 
    Depth maps are obtained by synthetic rendering. & 
    Depth maps are reconstructed from point clouds, needing masks for invalid areas. & 
    Depth maps are obtained by twin digital synthetic rendering. \\
    \hline
\end{tblr}
\caption{\small Summary of Datasets \TODO{Make this table concise and smaller. Try to fit into one column. You don't need to write full sentence in each cell}}
\label{tab:data_sum}
\end{table*}

==> tables/edge_runtime.tex <==

\begin{table}[]
\centering
\resizebox{0.3\textwidth}{!}{%
\begin{tabular}{crr|rr}
\hline
\multicolumn{1}{l}{}              & \multicolumn{2}{c|}{\textbf{Orin Nano}}  & \multicolumn{2}{c}{\textbf{Snapdragon}}  \\ \cline{2-5} 
\multicolumn{1}{l}{} & \multicolumn{1}{c}{CPU} & \multicolumn{1}{c|}{GPU} & \multicolumn{1}{c}{CPU} & \multicolumn{1}{c}{GPU} \\ \hline
\multicolumn{1}{c|}{\textbf{Argos} (CVPR 2023) }        & \multicolumn{1}{r}{8774} & 209 & \multicolumn{1}{r}{1424} & 914 \\ \hline
\multicolumn{1}{c|}{\textbf{MulHeadDepth} (Ours)} & \multicolumn{1}{r}{\textbf{6183}} & 216 & \multicolumn{1}{r}{\textbf{1156}} & \textbf{617} \\ \hline
\multicolumn{1}{c|}{\textbf{HomoDepth} (Ours)}   & \multicolumn{1}{r}{6611} & \textbf{203} & \multicolumn{1}{r}{1512} & 893 \\ \hline
\end{tabular}%
}
\vspace{-3mm}
\caption{\small \textbf{Latency of models in millisecond} on NVIDIA\textregistered ~Jetson Orin Nano\texttrademark~ Developer Kit and Snapdragon 8+ Gen 1 Platform}
\label{tab:edge_res}
\vspace{-6mm}
\end{table}
